Training Hamiltonian neural networks without backpropagation

Neural networks that synergistically integrate data and physical laws offer great promise in modeling dynamical systems. However, iterative gradient-based optimization of network parameters is often computationally expensive and suffers from slow convergence. In this work, we present a backpropagation-free algorithm to accelerate the training of neural networks for approximating Hamiltonian systems through data-agnostic and data-driven algorithms. We empirically show that data-driven sampling of the network parameters outperforms data-agnostic sampling or the traditional gradient-based iterative optimization of the network parameters when approximating functions with steep gradients or wide input domains. We demonstrate that our approach is more than 100 times faster with CPUs than the traditionally trained Hamiltonian Neural Networks using gradient-based iterative optimization and is more than four orders of magnitude accurate in chaotic examples, including the H\'enon-Heiles system.

==> sections/relwork.tex <==


\section{Related work}\label{section:related-work}


%To learn the dynamics of Hamiltonian systems from data using neural networks, Hamilton's equations
%have been integrated into the network's loss formulation \citep{greydanus-2019-HNN, bertalan-2019}.
%Studies have taken different directions to capture the dynamics of Hamiltonian systems;
%one focuses on learning the Hamiltonian function of an underlying system, and the other on
%learning the time evolution of the system by learning the flow map.

%\paragraph{Neural Ordinary Differential Equation}


\paragraph{Hamiltonian neural networks (HNNs)} \label{section:related-work:hamiltonian-neural-networks}
Hamilton's equations have been incorporated into the network's loss formulation by \citet{greydanus-2019-HNN}
and \citet{bertalan-2019} in order to learn the conserved quantities of the system. In both independent studies
the loss is operated on the gradient of the network's output with respect to inputs, and both resort
to traditional gradient-based network training methods and automatic differentation to compute the
gradients.
%The authors show that HNN conserves an energy-like quantity, whereas the baseline model does not. Additionally, when predicting the trajectories on the well-trained HNN, the study shows that HNN could better predict the trajectories than the baseline model \cite{greydanus-2019-HNN}.
%%Note that while the output of the HNN does have a conserved "energy-like" quantity, it does not resemble the true Hamiltonian of the system and, therefore, is not the real conserved property of the system. To note, when a pinning term is assumed to be known, then HNN output can be correctly shifted and can approximate the exact Hamiltonian function \cite{bertalan-2019}.
%Recent research have focused on variations of HNNs
%\citep{han-2021-adaptable-HNNs, shaan-2021-port-HNN, sosanya-2022-dissipative-HNN, khoo-2023-separable-HNN}.
Later many variations have been studied including adaptable HNNs \citep{han-2021-adaptable-HNNs},
which incorporate an input channel -- a bifurcation parameter -- for approximating a parametrized
Hamiltonian function, port HNNs \citep{shaan-2021-port-HNN} for controlling force, dissipative HNNs
\citep{sosanya-2022-dissipative-HNN} for dissipative systems, and separable HNNs which incorporate
separability of the Hamiltonian into the network architecture \citep{khoo-2023-separable-HNN}.
%that makes the trained model adaptable to parameter variations of the Hénon-Heiles system.
%Port HNNs additionally incorporate a separate network that depends on time \(t\) for controlling force
%\citep{shaan-2021-port-HNN}. Dissipative HNNs for dissipative Hamiltonian systems include an additional
%sub-network that outputs Rayleigh dissipation to account for dissipative effects \citep{sosanya-2022-dissipative-HNN}.
%Separable HNNs incorporate additive separability into the network architecture as an inductive bias
%\citep{khoo-2023-separable-HNN}.


The authors of \citep{bertalan-2019} have additionally demonstrated Gaussian processes by solving
an associated fully linear system incorporating Hamilton's equations. They use kernel functions to
construct the basis functions for the approximation. Inspired by this linear system we use neural network
activation functions as the basis functions in our framework.


\paragraph{HNNs with symplectic integrators}\label{section:related-work:hamiltonian-neural-networks-with-symplectic-integrators}
Using time series data of position \(q\) and and momentum \(p\) only, one can train HNN by relying on
the finite differences, as mentioned in \citep{greydanus-2019-HNN}. This would give rise to forward
Euler integration scheme in the HNN's objective and remove the requirement for derivative information
in the network training. Many recent studies focus on this numerical integration of HNN, including
symplectic recurrent neural networks (SRNNs) introduced by \citet{chen-2019-SRNNs}, outperforming HNN in
long-term trajectory predictions using a higher-order Leapfrog integration scheme \citep{leimkuhler-2004-simulating-hamiltonian-dynamics-leapfrog-symplectic, hairer-2006-geometric-numerical-integration-also-symplectic}
splitting the network into kinetic and potential energy parts. Therefore they can only considering separable
systems. The authors report that the networks predictions even outperforms trajectories simulated
by the exact Hamiltonian equations. This may be because the network learns to minimize the numerical
error made by the integrator \citep{chen-2019-SRNNs, horn-2022}. Symplectic ordinary differential equations (ODE)-Net
(SymODEN)
and its dissipative variation also learn with an integrated numerical integrator but can additionally
account for external force, e.g., control \citep{zhong-2020-symoden, zhong-2020-dissipative-symoden}.
%Inspired by SymODEN, capturing SE(3) kinematics for robotic applications are studied in \citep{duong-2021-hnode-robotics}.
Using an extended explicit high-order integrator scheme \citet{xiong-2022-nonseperable-symplectic-NNs}
use an extended phase space to also handle non-separable Hamiltonians. Since all the above mentioned
methods utilize backpropagation through an integrator using a gradient based training method, their
training is reportedly more time consuming \citet{xiong-2022-nonseperable-symplectic-NNs}. SympNet
is developed to directly approximate symplectic maps \citet{jin-2020-sympnets}. The authors note that
training is much faster than HNN methods and outperforms them in trajectory prediction, however, due to
number of parameters in SympNet it is hard to scale it to higher dimensional problems. Motivated by
SympNet, TaylorNet is introduced for separate systems \citet{tong-2021-taylornet}.

\paragraph{Random feature models for Hamiltonian approximation}
Random features have been used for learning Hamiltonian flow \citet{tanaka-2022-symplectic-spectrum-GPs, jakovac-2022}.
 \citep{tanaka-2022-symplectic-spectrum-GPs} use Gaussian processes with symplectic random Fourier features
 integrated with Hamiltonian mechanics, and \citep{jakovac-2022} use extreme learning machines (ELMs),
 which both are data-agnostic sampling schemes.



%\paragraph{Other architectures}\label{section:related-work:other-architectures}
%Lagrangian neural networks \citep{cranmer-2020-LNNs} use the Lagrangian formalism instead of the
%Hamiltonian as the physical bias. Learning a symplectic reduced-order Hamiltonian \citep{sharma-2022, yildiz-2023},
%and learning coordinate-free symplectic 2-form from data \citep{chen-2021-neural-symplectic-form} has
%been studied as well.


%\paragraph{Error analysis and correction}\label{section:related-work:error-analysis-and-correction}
%\citep{zhu-2020-HNN-with-midpointrule} theoretically analyze the trainig of HNNs using finite differences
%with symplectic and non-symplectic integration schemes. Using symplectic integrators, the predicted
%trajectories (network tragets) have higher accuracy; conversly, the networks trained with symplectic
%integrator schemes learn the network targets rather than the real Hamiltonian. Their work aligns with
%the numerical results in \citet{chen-2019-SRNNs}, where the trained network accounts for the numerical
%errors. An adapted loss is proposed in \citet{zhu-2020-HNN-with-midpointrule} to learn inverse modified
%Hamiltonians. Similarly, the Gaussian process demonstrated by \citet{bertalan-2019} has been extended
%to learn the inverse-modified Hamiltonian. In an independent study, \citep{david-2023} confirm that no
%exact Hamiltonian can be learnt only from time series data by HNN due to integration errors. Similar to
%\citep{zhu-2020-HNN-with-midpointrule}, the authors use the formal series expansion of the HNN output
%trained with symplectic integrators and porpose a post-training correction step to the HNN output
%to recover the original Hamiltonian of the system. We adapt the proposed post-training correction
%scheme and demonstrate that it can also be applied to our framework.



